Adaptive CPU Resource Allocation for Emulator in Kernel-based Virtual Machine

The technologies of heterogeneous multi-core architectures, co-location, and virtualization can be used to reduce server power consumption and improve system utilization, which are three important technologies for data centers. This article explores the scheduling strategy of Emulator threads within virtual machine processes in a scenario of co-location of multiple virtual machines on heterogeneous multi-core architectures. In this co-location scenario, the scheduling strategy for Emulator threads significantly affects the performance of virtual machines. This article focuses on this thread for the first time in the relevant field. This article found that the scheduling latency metric can well indicate the running status of the vCPU threads and Emulator threads in the virtualization environment, and applied this metric to the design of the scheduling strategy. This article designed an Emulator thread scheduler based on heuristic rules, which, in coordination with the host operating system's scheduler, dynamically adjusts the scheduling scope of Emulator threads to improve the overall performance of virtual machines. The article found that in real application scenarios, the scheduler effectively improved the performance of applications within virtual machines, with a maximum performance improvement of 40.7%.

==> figures/flow_chart.tex <==

% 定义流程图节点
\tikzstyle{startstop} = [
  rectangle,
  rounded corners,
  minimum width=2cm,
  minimum height=1cm,
  text centered,
  draw=black
]
\tikzstyle{io} = [
  trapezium,
  trapezium left angle=75,
  trapezium right angle=105,
  minimum width=1cm,
  minimum height=1cm,
  text centered,
  draw=black
]
\tikzstyle{process} = [
  rectangle,
  minimum width=2cm,
  minimum height=1cm,
  text centered,
  draw=black
]
\tikzstyle{decision} = [
  diamond,
  minimum width=2cm,
  minimum height=1cm,
  text centered,
  draw=black]
\tikzstyle{arrow} = [thick, ->, >=stealth]

\begin{tikzpicture}[node distance=2cm]
  % 设置节点
  \node (pic) [startstop] {待测图片};
  \node (bg) [io, below of=pic] {读取背景};
  \node (pair) [process, below of=bg] {匹配特征点对};
  \node (threshold) [decision, below of=pair, yshift=-0.5cm] {多于阈值};
  \node (clear) [decision, right of=threshold, xshift=3cm] {清晰？};
  \node (capture) [process, right of=pair, xshift=3cm, yshift=0.5cm] {重采};
  \node (matrix_p) [process, below of=threshold, yshift=-0.8cm] {透视变换矩阵};
  \node (matrix_a) [process, right of=matrix_p, xshift=3cm] {仿射变换矩阵};
  \node (reg) [process, below of=matrix_p] {图像修正};
  \node (return) [startstop, below of=reg] {配准结果};
    
  % 连接节点
  \draw [arrow](pic) -- (bg);
  \draw [arrow](bg) -- (pair);
  \draw [arrow](pair) -- (threshold);

  \draw [arrow](threshold) -- node[anchor=south] {否} (clear);

  \draw [arrow](clear) -- node[anchor=west] {否} (capture);
  \draw [arrow](capture) |- (pic);
  \draw [arrow](clear) -- node[anchor=west] {是} (matrix_a);
  \draw [arrow](matrix_a) |- (reg);

  \draw [arrow](threshold) -- node[anchor=east] {是} (matrix_p);
  \draw [arrow](matrix_p) -- (reg);
  \draw [arrow](reg) -- (return);
\end{tikzpicture}

